Financial Markets Prediction with Deep Learning

Financial markets are difficult to predict due to its complex systems dynamics. Although there have been some recent studies that use machine learning techniques for financial markets prediction, they do not offer satisfactory performance on financial returns. We propose a novel one-dimensional convolutional neural networks (CNN) model to predict financial market movement. The customized one-dimensional convolutional layers scan financial trading data through time, while different types of data, such as prices and volume, share parameters (kernels) with each other. Our model automatically extracts features instead of using traditional technical indicators and thus can avoid biases caused by selection of technical indicators and pre-defined coefficients in technical indicators. We evaluate the performance of our prediction model with strictly backtesting on historical trading data of six futures from January 2010 to October 2017. The experiment results show that our CNN model can effectively extract more generalized and informative features than traditional technical indicators, and achieves more robust and profitable financial performance than previous machine learning approaches.

==> criterion.tex <==
\section{Criterion}

\subsection{From Finance's Viewpoint}
Previous researches usually choose buy-and-hold strategy as the baseline, however, we find that this strategy is too conservative to evaluate current models' performance. Take the future CL for instance, if we placed and held one contract of this future and levered it 1000 times since July, 2014, our assert so far would shrink around 70000 dollars.  In our research, we choose two classic models, SVM and NN, as our research's baselines, which are used to predict stock market by \cite{kim2003financial} and \cite{fernandez2003technical}, respectively. Moreover, as the benchmark in financial field, the backtest strategy we using is stricter than \cite{dixon2016classification,fernandez2003technical}: we set an expensive transaction fee over real-life trading to keep our backtest result under conservative scenario:

%we define positive return as the first-level criterion to evaluate our MLP model's performance; further we define our MLP model's performance as second-level criterion for our other models; moreover, as the benchmark of financial return, the backtest strategy we using is more strict than \cite{dixon2016classification, rechenthin2014machine}: we set following fees to keep our backtest result under conservative scenario:

\begin{equation}
C = 2 + 2 \left( I * M\right)
\end{equation}
\begin{equation}
S = 5 \left(I * M\right) 
\end{equation}
\begin{equation}
T = 2\left(C + S\right)
\end{equation}

Where $C$ is denoted as $Commission$, $S$ is denoted as $Slippage$, $I$ is denoted as $Increment of Price$, $M$ is denoted as $Leverage Multiplier$, and $T$ is denoted as $Transaction Fee$.

It means that, if the Increment of Price is 0.01 and Leverage Multiplier is 1000, one contract's profit needs to gain no less than 144 dollars; otherwise, this contract will end up losing money. The specification of our backtest strategy is shown as follow(auxiliary parts not included, such as Sharpe Ratio and Drawdown):
\begin{itemize}
\item The input file of the test is a CSV format file, the columns of which consist of ``Date Time", ``Open Price", ``Close Price" and ``Prediction Label"($PL$), the rows of which are time series at two-hour intervals and at ascending order of "Date Time".
\item At the initial stage of the test, initialize all the arguments, which include Initial Capital($Cap$), Leverage Multiplier($M$), Increment of Price($I$), Transaction Fee($T$),  and Current Trading State($CS$).
\item The profit by Short Trade is equal to:
\begin{equation}
PT_{s} = \left(P_{oe} - P_{ol}\right) *  M - T
\end{equation}
Where $PT_{s}$ is denoted the profit by Short Trade, $P_{oe}$ is the open price at the contract entering the market, $P_{ol}$ is the open price at the contract leaving the market.
\item The profit by Long Trade is equal to:
\begin{equation}
PT_{l} = \left(P_{ol} - P_{oe}\right) *  M - T
\end{equation}
Where $PT_{l}$ is denoted the profit by Long Trade.
\item Scan each row in chronological order:
	\begin{itemize}
		\item $CS$ enters in ``In Long Trade" if $CS$ is ``Idle" and $PL$ is ``Up".
		\item $CS$ enters in ``In Short Trade" if $CS$ is ``Idle" and $PL$ is `Down".
		\item $Cap$ incremented by $PT_{s}$ and $CS$ enters in ``In Long Trade", if $CS$ is ``In Short Trade" and $PL$ is ``Up".
		\item $Cap$ incremented by $PT_{l}$  and $CS$ enters in ``In Short Trade", if $CS$ is ``In Long Trade" and $PL$ is ``Down".
		\item $Cap$ incremented by $PT_{s}$ and then returned, if $CS$ is ``In Short Trade" and current row is the last one.
		\item $Cap$ incremented by $PT_{l}$ and then returned, if $CS$ is ``In Long Trade" and current row is the last one.
		\end{itemize}
\end{itemize}

%Algorithm ~\ref{alg-bt} summarizes the procedure for our backtest stradety(not including auxiliary parts, such as Sharpe Ratio and Drawdown).



%\begin{algorithm}
%\caption{Backtest Basic Flow}
%\label{alg-bt}
%\begin{algorithmic}
%\REQUIRE 
%\begin{tabular}[t]{@{}l}
%Initial Capital, Time Series with Date Time, \\
%Open Price, Close Price and Predicting Label
% \end{tabular}
%\ENSURE  Final Capital \\
%%\COMMENT Defining parameters
%%\STATE
%%	$\text{Commission Fee} \gets 2 + 2 \left( \text{Increment of Price} * \text{Leverage Multiplier} \right)$\\
%%	$\text{Slippage} \gets 5 \left(\text{Increment of Price} * \text{Leverage Multiplier}\right)$ \\
%%	$\text{Transaction Fee} \gets \text{Slippage} + \text{Commission Fee}$ \\
%%	$\text{In Long Trade} \gets False$ \\
%%	$\text{In Short Trade} \gets False$ \\
%%	$\text{Final Capital} \gets \text{Initial Capital}$ \\
%	
%\begin{itemize}
%\item Initialization
%	\begin{itemize}
%		\item Define Capital to 100000 dollars
%		\item Define Leverage Multiplier
%		\item Define Increment of Price
%		\item Define Commission Fee as Formula 3
%		\item Define Slippage as Formula 4
%		\item Define Transaction Fee as the 2 times of sum of Commission Fee and Slippage
%		\item Define Number of Contracts to 1 
%		\item Define Current Status to Idle
%	\end{itemize}
%		
%%		\item \COMMENT Preprocess Prediction Series \\
%%		For each line of prediction series as the ordering of Datetime:
%%		\begin{itemize}
%%			\item Prediction changes to Up
%%			\begin{itemize}
%%				\item if Prediction is Flat and the previous Prediction is Up
%%			\end{itemize}
%%			\item Prediction changes to Down
%%			\begin{itemize}
%%				\item if Prediction is Flat and the previous Prediction is Down
%%			\end{itemize}
%%			\item Prediction no change
%%			\begin{itemize}
%%				\item other cases
%%			\end{itemize}
%%		\end{itemize}
%%	\end{itemize}
%
%%\COMMENT Calculate profit row by row
%
%\item FOR each line of prediction series as the ordering of Datetime:
%    \begin{itemize}
%    \item Current Status is set to In Long Trade
%    	\begin{itemize}
%		\item if Prediction is Up
%		\item if Prediction is Flat and Current Status is In Long Trade
%	\end{itemize}
%    \item Current Status is set to In Short Trade
%    	\begin{itemize}
%		\item if Prediction is Down
%		\item if Prediction is Flat and Current Status is In Short Trade
%	\end{itemize}
%    \end{itemize}
%    
%    \begin{itemize}
%    \item  Capital No Change
%        	\begin{itemize}
%        		\item If Prediction is Flat and Current Status is neither In Long Trade nor In Short Trade
%      		\item If Prediction is not Down and Current Status is In Long Trade
%        		\item if Prediction is not Up and Current Status is In Short Trade
%        	\end{itemize}
%  
%    \item  \COMMENT Long Transaction may be negative \\
%    Capital incremented by Long Transaction = Open Price Change * Leverage Multiplier - Transaction Fee
%    	\begin{itemize}
%    		\item if this is the last prediction and Current Status is In Long Trade
%    		\item if Prediction is Down and Current Status is In Long Trade
%    	\end{itemize}
%   
%    \item  \COMMENT Short Transaction may be negative \\
%    Capital incremented by Short Transaction = Open Price Change * Leverage Multiplier - Transaction Fee
%    	\begin{itemize}
%    		\item if this is the last prediction and Current Status is In Short Trade
%    		\item if Prediction is Long and Current Status is In Short Trade
%    	\end{itemize}
%    \end{itemize}	
%\end{itemize}
%%\COMMENT Substitute intermediate Flat labels with previous Non-Flat one
%%\FOR {Each row of Time Series along the order of Date Time}
%%\IF {Predicting Label $is$ $Flat$ \AND Predicting Label is in the first row}
%%%\IF {Predicting Label $is$ $Flat$}
%%	\STATE
%%		$\text{Predicting Label} \text{ } No \text{ } Change$ \\
%%		$\text{Previous Label} \gets Flat$
%%\ELSE
%%	\IF {$\text{Predicting Label} \text{ } is \text{ } Flat$}
%%		\STATE
%%			$\text{Predicting Label} \gets \text{Previous Label}$
%%	\ELSE
%%		\STATE
%%			$\text{Predicting Label} \text{ } No \text{ } Change$ \\
%%			$\text{Previous Label} \gets \text{Predicting Label}$
%%	\ENDIF
%%\ENDIF
%%\ENDFOR \\
%%\algstore{alg-bt}
%%\end{algorithmic}
%%\end{algorithm}
%%
%%\begin{algorithm}                     
%%\begin{algorithmic}[1]
%%\algrestore{alg-bt}
%
%%\FOR {Each row of Time Series along the order of Date Time}
%%	\IF {($\text{Predicting Label} \text{ } is \text{ } Flat$ \AND $\text{In Long Trade} \text{ } is \text{ } False$ \AND $\text{In Short Trade} \text{ } is \text{ } False$) \OR \\
%%	 ($\text{Predicting Label} \text{ } is \text{ } Up$ \AND $\text{In Long Trade} \text{ } is \text{ } True$) \OR \\
%%	 ($\text{Predicting Label} \text{ } is \text{ } Down$ \AND $\text{In Short Trade} \text{ } is \text{ } True$)}
%%		\STATE $No \text{ } change$
%%	\ELSE
%%		\IF {$EOF$ \AND $\text{In Long Trade} \text{ } is \text{ } True$}
%%			\STATE
%%				$\text{Long Transaction} \gets \text{Number of Contracts} * \text{Open Price} - \text{Transaction Fee}$ \\
%%				$\text{Final Capital} \gets \text{Final Capital} + \text{Long Transaction}$ \\
%%				\RETURN $\text{Final Capital}$
%%		\ELSIF {$EOF$ \AND In Short Trade $is$ $True$}
%%			\STATE
%%				$\text{Short Transaction} \gets \text{Number of Contracts} * \text{Open Price} + \text{Transaction Fee}$ \\
%%				$\text{Final Capital} \gets \text{Final Capital} - \text{Long Transaction}$ \\
%%				\RETURN $\text{Final Capital}$
%%		\ELSIF {Predicting Label $is$ $Up$ \AND In Short Trade $is$ $True$}
%%			\STATE
%%				 $\text{Short Transaction} \gets \text{Number of Contracts} * \text{Open Price} + \text{Transaction Fee}$ \\
%%				 $\text{Long Transaction} \gets \text{Number of Contracts} * \text{Open Price} + \text{Transaction Fee}$ \\
%%				 $\text{Final Capital} \gets \text{Final Capital} - \text{Short Transaction} - \text{Long Transaction}$ \\
%%				 $\text{In Short Trade} \gets False$ \\
%%				 $\text{In Long Trade} \gets True$
%%		\ELSIF {Predicting Label $is$ $Down$ \AND In Long Trade $is$ $True$}
%%			\STATE
%%				 $\text{Short Transaction} \gets \text{Number of Contracts} * \text{Open Price} - \text{Transaction Fee}$ \\
%%				 $\text{Long Transaction} \gets \text{Number of Contracts} * \text{Open Price} - \text{Transaction Fee}$ \\
%%				 $\text{Final Capital} \gets \text{Final Capital} + \text{Short Transaction} + \text{Long Transaction}$ \\
%%				 $\text{In Short Trade} \gets True$ \\
%%				 $\text{In Long Trade} \gets False$
%%		\ELSIF {Predicting Label $is$ $Up$ \AND In Long Trade $is$ $False$ \AND In Short Trade $is$ $False$}
%%			\STATE
%%				$\text{Long Transaction} \gets \text{Number of Contracts} * \text{Open Price} + \text{Transaction Fee}$ \\
%%				$\text{Final Capital} \gets \text{Final Capital} - \text{Long Transaction}$ \\
%%				$\text{In Long Trade} \gets True$
%%		\ELSIF {Predicting Label $is$ $Down$ \AND In Long Trade $is$ $False$ \AND In Short Trade $is$ $False$}
%%			\STATE
%%				$\text{Short Transaction} \gets \text{Number of Contracts} * \text{Open Price} - \text{Transaction Fee}$ \\
%%				$\text{Final Capital} \gets \text{Final Capital} + \text{Long Transaction}$ \\
%%				$\text{In Short Trade} \gets True$
%%		\ENDIF
%%	
%%	\ENDIF
%%\ENDFOR
%
%\end{algorithmic}
%\end{algorithm}


\subsection{From Machine Learning's Viewpoint}
The regular evaluating metrics in machine learning field, such as F1 score and accuracy, is ineffective to this research as well. As shown in our backtest strategy, the $Up$ and $Down$ class play vital roles in the backtest process: the first $Up$ or $Down$ label renders $Capital$ into the market; the turning point of $Up$ and $Down$ renders $Capital$ ending current trade and then entering next trade. During this process, the $Flat$ label only holds current status. Thus, wrong labels can be classified to 3 levels as the order of severity: the first-level wrong labels are the "reversed" $Up$ or $Down$ labels, which is directly opposite with trends thus to bring double loss; the second-level wrong labels are the $Flat$ labels that are predicted $Up$ or $Down$ falsely, this type of errors usually lead to moderate loss such as $Transaction Fee$; the third-level wrong labels are the $Up$ or $Down$ labels that are predicted $Flat$ falsely---in this case, we only loss the chances gaining profit. On the other hand, the importance of true labels is different as well: The true $Up$ and $Down$ labels are much important than the true $Flat$.

Therefore, we propose a modified version of F score according to the aforementioned analysis, which is similar as the original F score for Type I and Type II errors, however, we use the aforementioned the First-level, Second-level and Third-level Errors instead:

\begin{equation}
N_{tp} = N_{tu} + N_{td} + \beta_{3}^2N_{tf}
%\text{True Positive} = \text{Number of True $Up$} + \text{Number of True $Down$} 
\end{equation}
\begin{equation}
E_{1st} = E_{wutd} + E_{wdtu}
%\text{First-level Errors} = \text{Number of Wrong $Up$ but True $Down$} + \text{Number of Wrong $Down$ but True $Up$}
\end{equation}
\begin{equation}
E_{2nd} = E_{wutf} + E_{wdtf}
%\text{Second-level Errors} = \text{Number of Wrong $Up$ but True $Flat$} + \text{Number of Wrong $Down$ but True $Flat$}
\end{equation}
\begin{equation}
E_{3rd} = E_{wftu} + E_{wftd}
%\text{Third-level Errors} = \text{Number of Wrong $Flat$ but True $Up$} + \text{Number of Wrong $Flat$ but True $Down$}
\end{equation}
\begin{equation}\label{eqn:FS}
F = \frac{\left(1+\beta_{1}^2+\beta_{2}^2\right)N_{tp}}{\left(1+\beta_{1}^2+\beta_{2}^2\right)N_{tp}+E_{1st}+\beta_{1}^2E_{2nd}+\beta_{2}^2E_{3rd}}
%\text{F1 Score} = \frac{\left(1+\beta_{1}^2+\beta_{2}^2\right)\text{True Positive} }{\left(1+\beta_{1}^2+\beta_{2}^2\right)\text{True Positive}+\text{First-level Errors}+\beta_{1}^2\text{Second-level Errors}+\beta_{2}^2\text{Third-level Errors}}
\end{equation}
where $N_{tp}$ is denoted as True Positive, $E_{1st}$ is denoted as First-level Errors, $E_{2nd}$ is denoted as Second-level Errors, $E_{3rd}$ is denoted as Third-level Errors, $N_{tu}$ is denoted as True Up, $N_{td}$ is denoted as True Down, $N_{tf}$ is denoted as True Flat, $E_{wutd}$ is denoted as Wrong Up but True Down, $E_{wdtu}$ is denoted as Wrong Down but True Up, $E_{wutf}$ is denoted as Wrong Up but True Flat, $E_{wdtf}$ is denoted as Wrong Down but True flat, $E_{wftu}$ is denoted as Wrong Flat but True Up, $E_{wftd}$ is denoted as Wrong Flat but True Down. $\beta_{1}$ and $\beta_{2}$ are denoted as the weighting parameters for Second-level and Third-level Errors, respectively. In our research, we set $\beta_{1}$ to 0.5, $\beta_{2}$ and $\beta_{3}$ to 0.125.






==> data.tex <==
\section{Data}

The datasets we used in this study are historical trading data of commodity futures from January 2010 to ??? 2017, including Crude Oil (CL), ..., ???. The timing interval between two adjacent trading records is five minutes, and each record has the following seven attributes: date, time, open price, high price, low price, close price, and trading volumes. Note that these are fundamental information for trading activites of a financial instrument, and the open-high-low-close chart (OHLC) is often used to illustrate movements in the price of a financial instrument over time.  

Technical indicators are a fundamental part of technical analysis, which has been widely used to analyze securities and make investment decisions. A large variety of technical indicators have been developed to predict the future price levels, or simply the general price direction, of a security by looking at past patterns. We choose technical indicators according to their functionality and popularity. For lagging indicators, which are often used to identify and confirm the strength of a pattern or trend, we pick Expotential Moving Average (EMA), Moving Average Convergence Divergence (MACD) Histogram, Bollinger Band. For leading indicators, which usually change before a trend or pattern and are thus used during periods of sideways or non-trending ranges, we pick Relative Strength Index (RSI),  Commodity Channel Index (CCI), Volume Weighted Average Price (VWAP), On-balance Volume (OBV), Average Directional Index (ADX), Accumulation Distribution Line (ADL), and Chaikin Money Flow (CMF). In addition, we also include technical indicators regarded as neither lagging nor leading indicators such as Rate of Change (ROC). Different time spans are used to generate EMA, MACD Histogram, Bollinger Band, ROC, RSI, CCI, CMF and ADX. Together with the original five attributes (open, high, low, close prices, and trading volumes), each data point has a total number of 46 attributes.

Our model predicts the commodity price movement every two hours and makes the trading decisions accordlying based on the prediction outcome. The reason that our model works with a two-hour time interval is two folds:

\begin{enumerate}
	\item Longer time intervals provide necessarily data sequence size for convolution. Each 24 consecutive five-minute data points are organized to form a data frame, where 1-D convolution is applied along the time-line. For example, a kernal of size 3x1 applied on the data frame will produce a 8x1 activation map in the resulting convolution layer. For the sake of fair comparisons between our MLP and CNN models, the datasets fed to the MLP model also have the same time interval. More details about our CNN model are described in Section \ref{sec:?}.
	
	\item The price change of a commodity over a shorter time interval is usually much smaller than that over a longer time interval. For example, the average price change of CL over a five-minutes time interval is ?? compared to ??? over a two-hour time interval. The profitability of trading over short time intervals is thus diminished after slippage and transactions fees are applied. 
	
%	Longer time intervals make dataset balanced more easily. in 5-minute time scale, There are the overwhelming majority of data candles whose price change compared to the previous one is even smaller than transaction fee. If these data candles are labeled Up or Down, then they may be still negative trades even though they are correctly predicted.


\end{enumerate}

Another vital part of our data pre-processing is labeling. The popular way for labeling stock or commodity price movement is based on a fixed threshold for the log return of the price, i.e., the data point at time $t$ is marked as "going up" or "going down" if the log return of the price at time $t+1$ over $t$ is above or below the pre-specified threshold. However, because the aforementioned method does not well consider the distribution of future price's trend \cite{lopez20177}, we adopt the dynamic threshold method as described in \cite{sun2017predicting}:

\begin{equation}
l_{t+1} =
\begin{cases}
\text{up,}      & \text{if $c_{t+1} \geq c_{t} \left( 1 + \alpha v_{t}\right)$} \\
\text{down,}  & \text{if $c_{t+1} \leq c_{t} \left( 1 - \alpha v_{t}\right)$} \\
\text{flat,}     & \text{Otherwise}
\end{cases}
\end{equation}
where $c_{t}$ and $v_{t}$ represent the close price and volatility of a commodity price at time $t$, and $\alpha$ is a parameter that can be adjusted to balance the three classes. In our study, the volatility is measured by using the standard deviation of the past ten data points of any given time, and $\alpha$ is set to be 0.55.

